Need for Sleep: the Impact of a Night of Sleep Deprivation on Novice Developers' Performance

We present a quasi-experiment to investigate whether, and to what extent, sleep deprivation impacts the performance of novice software developers using the agile practice of test-first development (TFD). We recruited 45 undergraduates and asked them to tackle a programming task. Among the participants, 23 agreed to stay awake the night before carrying out the task, while 22 slept usually. We analyzed the quality (i.e., the functional correctness) of the implementations delivered by the participants in both groups, their engagement in writing source code (i.e., the amount of activities performed in the IDE while tackling the programming task) and ability to apply TFD (i.e., the extent to which a participant can use this practice). By comparing the two groups of participants, we found that a single night of sleep deprivation leads to a reduction of 50% in the quality of the implementations. There is important evidence that the developers' engagement and their prowess to apply TFD are negatively impacted. Our results also show that sleep-deprived developers make more fixes to syntactic mistakes in the source code. We conclude that sleep deprivation has possibly disruptive effects on software development activities. The results open opportunities for improving developers' performance by integrating the study of sleep with other psycho-physiological factors in which the software engineering research community has recently taken an interest in.

==> RelatedWork.tex <==
\section{Related Work}\label{sec:Related}
\todo[author=Giuseppe,inline,color=cyan]{I'know that Davide made a deep study on Physiology and SE. There are also a couple of papers in the proceedings of the past ICSE proc. }
\subsection{Physiology in SE}
\subsection{Test-driven development}
Here we focus on productivity and process conformance.
Several quantitative studies have assessed the effectiveness of TDD, and the results of these studies have in turn been examined in a number of systematic reviews and meta-analyses~\cite{Munir:2014bp,rafique2012effects,turhan2010effective}.
The results of these analyses have been contradictory regarding both software products (e.g., defects) and  developers (e.g., productivity).
Interestingly, one of the secondary studies~\cite{CausevicSP11} suggested that \textit{insufficient adherence to the TDD protocol} and \textit{insufficient testing skills} are among the factors hampering industrial adoption of TDD.
Only a few studies have focused on the perception of developers regarding the TDD practice. 
For example, Mueller and Tichy~\cite{919128} examined several Agile methodologies, including TDD, within a university course and found that TDD was one of the most difficult techniques to adopt because developers felt that it was impractical to write test cases before coding. 
On the other hand, Gupta and Jalote~\cite{4343756} reported that students felt more confident that testing effort applied by using TDD would yield better results than a traditional test-after-code setting (test-last approach), while feeling the need for some upfront design.  
Pancur et al.~\cite{pancur2003} reported that students perceived TDD as more difficult for professionals to adopt. 
In particular, students perceived TDD as a practice that hindered their productivity, efficiency, and the quality of their code. 
Both students and professionals agreed that TDD helps in devising a better design and prevents bugs, but they also believed that this practice cannot replace a quality assurance engineer~\cite{ShullMTLDE10}. 
Even more interesting, participants also believed that the use of TDD improves confidence by minimizing the fear that existing parts of well-functioning source code would be compromised by the implementation of new features~\cite{1357925}.

